MaterialsAtlas.org: A Materials Informatics Web App Platform for Materials Discovery and Survey of State-of-the-Art

The availability and easy access of large scale experimental and computational materials data have enabled the emergence of accelerated development of algorithms and models for materials property prediction, structure prediction, and generative design of materials. However, lack of user-friendly materials informatics web servers has severely constrained the wide adoption of such tools in the daily practice of materials screening, tinkering, and design space exploration by materials scientists. Herein we first survey current materials informatics web apps and then propose and develop MaterialsAtlas.org, a web based materials informatics toolbox for materials discovery, which includes a variety of routinely needed tools for exploratory materials discovery, including materials composition and structure check (e.g. for neutrality, electronegativity balance, dynamic stability, Pauling rules), materials property prediction (e.g. band gap, elastic moduli, hardness, thermal conductivity), and search for hypothetical materials. These user-friendly tools can be freely accessed at \url{www.materialsatlas.org}. We argue that such materials informatics apps should be widely developed by the community to speed up the materials discovery processes.

==> extra.tex <==
We performed density functional perturbation theory (DFPT) calculations as implemented in VASP code for studying the mechanical properties of the predicted structures. The bulk, Shear, and Young's moduli  were calculated based on Hill approach \cite{Hill_1952}. For an infinitesimal strain ($\epsilon$) applied, the total energy of a given material can be computed using $E=E_0 + \frac{1}{2}V_0\sum_{i,j=1}^{6}C_{i,j}\epsilon_i\epsilon_j + O(\epsilon^3)$. Here, $C$ indicates the matrix of second-order elastic constants. If a material is mechanically stable, it should comply with the Born criteria. According to the Born elastic stability conditions,  the $C$ must be definite positive, all eigenvalues of $C$ metrix must be positive, and all the principal components must be positive. We employed VASPKIT \cite{VASPKIT} code to analyze the elastic properties, and mechanical stability of the structures. Furthermore, phonon dispersion relations were studied using phonopy code \cite{phonopy} to investigate the dynamical stability of the materials at 0K temperature.
